MetaMixer: A Regularization Strategy for Online Knowledge Distillation

Online knowledge distillation (KD) has received increasing attention in recent years. However, while most existing online KD methods focus on developing complicated model structures and training strategies to improve the distillation of high-level knowledge like probability distribution, the effects of the multi-level knowledge in the online KD are greatly overlooked, especially the low-level knowledge. Thus, to provide a novel viewpoint to online KD, we propose MetaMixer, a regularization strategy that can strengthen the distillation by combining the low-level knowledge that impacts the localization capability of the networks, and high-level knowledge that focuses on the whole image. Experiments under different conditions show that MetaMixer can achieve significant performance gains over state-of-the-art methods.

==> 2023_ICCV_maorongwang (2)/tab/depth.tex <==
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Network} & \multirow{2}{*}{\# of params} & \multirow{2}{*}{Baseline} & \multicolumn{2}{c}{MCL} & \multicolumn{2}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
{} & {}& {} & Avg. & Ens.& Avg. & Ens. \\
\midrule
ResNet-20 & 0.28M& 69.38&  70.80(+1.42) & 73.51(+4.13)   & 72.00(+2.62)& 73.41(+4.03)\\
ResNet-32 & 0.47M& 71.10&  72.70(+1.60) & 75.23(+4.13)   & 74.79(+3.69)& 76.45(+5.35)\\
ResNet-44 & 0.67M& 71.78&  73.85(+2.07) & 76.98(+5.20)   & 75.31(+3.53)& 77.43(+5.65)\\
ResNet-56 & 0.86M& 72.88&  74.49(+1.61) & 77.25(+4.37)   & 76.93(+4.05)& 78.70(+5.82)\\
ResNet-110& 1.74M& 74.14&  76.20(+2.06) & 78.26(+4.12)   & 78.58(+4.44)& 80.50(+6.36)\\
WRN-16-2  & 0.70M& 72.96& 74.51(+1.55)  & 76.73(+3.77)   & 76.40(+3.44)& 77.88(+4.92)\\
WRN-28-2  & 1.48M& 75.14& 76.83(+1.69)  & 78.82(+3.68)   & 79.04(+3.90)& 80.80(+5.66)\\
WRN-40-2  & 2.26M& 75.87& 77.55(+1.68)  & 79.69(+3.82)   & 80.18(+4.31)& 81.91(+6.04)\\
\bottomrule
\end{tabular}

==> 2023_ICCV_maorongwang (2)/tab/diffarch.tex <==
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
\multicolumn{2}{c}{Network} & \multicolumn{2}{c}{Baseline} & \multicolumn{3}{c}{DML} & \multicolumn{3}{c}{KDCL} & \multicolumn{3}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
Net 1 & Net 2 & Net 1 & Net 2 & Net 1 & Net 2 & Ens. & Net 1 & Net 2 & Ens. & Net 1 & Net 2 & Ens.  \\
\midrule
ResNet-20 & ResNet-32 &  92.76 & 93.46 & 92.91 & 93.50 & 93.87 & \underline{93.16}& \underline{93.82}& \underline{94.04}& \textbf{94.16} & \textbf{94.96} & \textbf{95.24}\\
ResNet-56 & ResNet-110&  94.08 & 94.47 & \underline{94.39} & \underline{94.88} & \underline{95.14} & 94.24& 94.49& 94.90& \textbf{95.76} & \textbf{96.19} & \textbf{96.40}\\
ResNet-32 & WRN-16-2  &  93.46 & 93.79 & 93.74 & 94.15 & 94.58 & \underline{94.21}& \underline{94.55}& \underline{94.81}& \textbf{95.14} & \textbf{95.17} & \textbf{95.59}\\
WRN-16-2 & WRN-28-2   &  93.79 & 94.94 & 94.47 & 95.05 & 95.27 & \underline{94.61}& \underline{95.43}& \underline{95.63}& \textbf{95.27} & \textbf{96.23} & \textbf{96.29}\\
WRN-16-2 & WRN-40-2   &  93.79 & 95.15 & 94.33 & 95.27 & 95.30 & \underline{94.53}& \underline{95.55}& \underline{95.78}& \textbf{95.31} & \textbf{96.54} & \textbf{96.44}\\
VGG-13-BN& WRN-16-2   &  94.23 & 93.79 & 94.57 & 94.15 & 95.03 & \underline{94.70} & \underline{94.33} & \underline{95.31} & \textbf{95.91} & \textbf{95.26} & \textbf{96.02}\\
\bottomrule
\end{tabular}
}

\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
\toprule
\multicolumn{2}{c}{Network} & \multicolumn{2}{c}{Baseline} & \multicolumn{3}{c}{DML} & \multicolumn{3}{c}{KDCL} & \multicolumn{3}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
Net 1 & Net 2 & Net 1 & Net 2 & Net 1 & Net 2 & Ens. & Net 1 & Net 2 & Ens. & Net 1 & Net 2 & Ens.  \\
\midrule
ResNet-20 & ResNet-32 & 69.38 & 71.10 & 70.37 & 72.49 & 73.52 & \underline{70.60} & \underline{72.84} & \underline{73.96} & \textbf{71.96} & \textbf{74.83} & \textbf{75.17}\\
ResNet-56 & ResNet-110& 72.88 & 74.14 & 74.03 & 75.82 & 76.67 & \underline{74.30} & \underline{75.92} & \underline{77.28} & \textbf{76.67} & \textbf{78.77} & \textbf{79.63}\\
ResNet-32 & WRN-16-2  & 71.10 & 72.96 & 72.83 & 74.09 & 75.38 & \underline{73.44} & \underline{74.74} & \underline{76.22} & \textbf{75.10} & \textbf{76.26} & \textbf{77.19}\\
WRN-16-2  & WRN-28-2  & 72.96 & 75.14 & 74.10 & 76.31 & 76.99 & \underline{75.06} & \underline{77.15} & \underline{78.53} & \textbf{76.21} & \textbf{79.02} & \textbf{79.38}\\
WRN-16-2  & WRN-40-2  & 72.96 & 75.87 & 74.17 & 77.44 & 77.81 & \underline{75.13} & \underline{78.09} & \underline{78.68} & \textbf{76.22} & \textbf{80.04} & \textbf{80.11}\\
VGG-13-BN & WRN-16-2  & 74.08 & 72.96 & 75.65 & 73.99 & 77.21 & \underline{77.21} & \underline{74.98} & \textbf{79.12} & \textbf{78.76} & \textbf{75.80} & \underline{78.87}\\
\bottomrule
\end{tabular}
}

==> 2023_ICCV_maorongwang (2)/tab/samearch.tex <==

\begin{table*}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{Network} & \multirow{2}{*}{Baseline} & \multicolumn{2}{c}{DML} & \multicolumn{2}{c}{ONE} & \multicolumn{2}{c}{KDCL} & \multicolumn{2}{c}{MCL} & \multicolumn{2}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
{} & {}& Avg. & Ens. & Avg. & Ens. & Avg. & Ens. & Avg. & Ens. & Avg. & Ens. \\
\midrule
ResNet-32 &  93.46  &  93.85  & 94.31  &  94.04  & 94.11 &  93.67  & 94.28  &  \underline{94.13} & \underline{94.74}   & \textbf{94.92} & \textbf{95.37}  \\
ResNet-56 &  94.08  &  94.25  & 94.80  &  \underline{94.72}  & 95.01 &  94.35  & 94.86  & 94.62  & \underline{95.06}   & \textbf{95.63} & \textbf{96.09} \\
ResNet-110&  94.47  &  94.61  & 95.00  &  \underline{95.14}  & \underline{95.45} &  94.39  & 94.93  & 94.86  & 95.37   & \textbf{96.07} & \textbf{96.44} \\
WRN-16-2  &  93.79  &  94.14  & 94.51  &  94.35  & \underline{94.74} &  \underline{94.45}  & 94.66  & 94.27  & 94.59   & \textbf{95.27} & \textbf{95.56}  \\
WRN-40-2  &  95.07  &  95.08  & 95.58  &  \underline{95.61}  & \underline{96.02} &  95.22  & 95.73  &  95.27 & 95.65   & \textbf{96.60} & \textbf{96.92}\\
VGG-13-BN &  94.23  &  94.63  & 95.09  &  \underline{94.74}  & 95.07 &  94.60  & 95.05  & 94.68 & \underline{95.11}  & \textbf{95.57} & \textbf{95.94}  \\
ShuffleNetV2 $\times$1 & 92.29 &  93.41  & 94.00  & 93.28  & 93.73 &  \underline{93.84}  & \underline{94.40}  &  93.07 & 93.61   & \textbf{93.96}& \textbf{94.55}\\
\bottomrule
\end{tabular}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{Network} & \multirow{2}{*}{Baseline} & \multicolumn{2}{c}{DML} & \multicolumn{2}{c}{ONE} & \multicolumn{2}{c}{KDCL} & \multicolumn{2}{c}{MCL} & \multicolumn{2}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
{} & {}& Avg. & Ens. & Avg. & Ens. & Avg. & Ens. & Avg. & Ens. & Avg. & Ens. \\
\midrule
ResNet-32 &  71.10  & 72.64   & 74.60  &  72.67  & 74.51 &  72.58  & 74.87  &  \underline{72.70} & \underline{75.23}   & \textbf{74.79} & \textbf{76.45}  \\
ResNet-56 &  72.88  & 74.13   & 75.99  &  \underline{76.51}  & 77.23 &  74.86  & 76.43  &  74.49 & \underline{77.25}   & \textbf{76.93} & \textbf{78.70}    \\
ResNet-110&  74.14  & 75.42   & 77.10  &  \underline{77.97}  & \underline{78.51} &  75.76  & 77.72  &  76.20 & 78.26   & \textbf{78.58} & \textbf{80.50}    \\
WRN-16-2  &  72.96  & 74.07   & 75.68  &  74.05  & 75.04 &  \underline{75.18}  & \underline{76.90}  &  74.51 & 76.73   & \textbf{76.40} & \textbf{77.88}    \\
WRN-40-2  &  75.87  & 77.35   & 79.15  &  \underline{79.04}  & \underline{80.23} &  78.02  & 79.85  &  77.55 & 79.69   & \textbf{80.18} & \textbf{81.91}    \\
VGG-13-BN &  74.08  & 75.74   & 77.12  &  75.93  & 77.06 &  77.01  & \underline{78.50}  &  \underline{77.02} & 78.42   & \textbf{78.28} & \textbf{79.47} \\
ShuffleNetV2 $\times$1& 72.52   & 74.66  & 76.34  & 74.31 & 75.57 & \underline{74.84}  & \underline{77.20} & 73.21 & 75.84 & \textbf{76.96} & \textbf{78.20}  \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Top-1 test accuracy (\%) compared with various online distillation methods on CIFAR-10 (top) and CIFAR-100 (bottom) dataset by training two networks with the same architecture. The baseline refers to the performance of the network when it is trained independently with only cross-entropy loss. Due to the special configuration of ONE, we regard the different branches as different networks. The \textit{Avg.} denotes the average performance of the models and \textit{Ens.} refers to the ensemble performance of two networks. Reported the average performance of three runs.}
\label{table:cifar-100}
\end{table*}

==> tab/depth.tex <==
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Network} & \multirow{2}{*}{\# of params} & \multirow{2}{*}{Baseline} & \multicolumn{2}{c}{MCL} & \multicolumn{2}{c}{MetaMixer (Ours)} \\
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
{} & {}& {} & Avg. & Ens.& Avg. & Ens. \\
\midrule
ResNet-20 & 0.28M& 69.38&  70.80(+1.42) & 73.51(+4.13)   & 72.00(+2.62)& 73.41(+4.03)\\
ResNet-32 & 0.47M& 71.10&  72.70(+1.60) & 75.23(+4.13)   & 74.79(+3.69)& 76.45(+5.35)\\
ResNet-44 & 0.67M& 71.78&  73.85(+2.07) & 76.98(+5.20)   & 75.31(+3.53)& 77.43(+5.65)\\
ResNet-56 & 0.86M& 72.88&  74.49(+1.61) & 77.25(+4.37)   & 76.93(+4.05)& 78.70(+5.82)\\
ResNet-110& 1.74M& 74.14&  76.20(+2.06) & 78.26(+4.12)   & 78.58(+4.44)& 80.50(+6.36)\\
WRN-16-2  & 0.70M& 72.96& 74.51(+1.55)  & 76.73(+3.77)   & 76.40(+3.44)& 77.88(+4.92)\\
WRN-28-2  & 1.48M& 75.14& 76.83(+1.69)  & 78.82(+3.68)   & 79.04(+3.90)& 80.80(+5.66)\\
WRN-40-2  & 2.26M& 75.87& 77.55(+1.68)  & 79.69(+3.82)   & 80.18(+4.31)& 81.91(+6.04)\\
\bottomrule
\end{tabular}
